Market Making via Reinforcement Learning

Market making is a fundamental trading problem in which an agent provides liquidity by continually offering to buy and sell a security. The problem is challenging due to inventory risk, the risk of accumulating an unfavourable position and ultimately losing money. In this paper, we develop a high-fidelity simulation of limit order book markets, and use it to design a market making agent using temporal-difference reinforcement learning. We use a linear combination of tile codings as a value function approximator, and design a custom reward function that controls inventory risk. We demonstrate the effectiveness of our approach by showing that our agent outperforms both simple benchmark strategies and a recent online learning approach from the literature.

==> src/tables/consolidated_ql.tex <==
\begin{table}[!ht]
    \centering
    \caption{}\label{tab:consolidated:ql}

    \begin{tabular}{
        l
        S[table-format=-1.2, table-figures-uncertainty=1,
        separate-uncertainty=true,table-align-uncertainty=true]
        S[table-format=3, table-figures-uncertainty=1,
        separate-uncertainty=true,table-align-uncertainty=true]
    }
        \toprule\toprule
        & {Daily Return [\%]} & {MAP [units]} \\
        \midrule
        \ticker{CRDI.MI} & -0.07 \pm 0.52 & 10 \pm 160 \\
        \ticker{GASI.MI} & -0.10 \pm 0.49 & 40 \pm 350 \\
        \ticker{GSK.L} & 0.24 \pm 0.53 & 50 \pm 540 \\
        \ticker{HSBA.L} & 0.40 \pm 0.64 & 120 \pm 660 \\
        \ticker{ING.AS} & -0.10 \pm 0.80 & 10 \pm 370 \\
        \ticker{LGEN.L} & 0.21 \pm 1.11 & 270 \pm 1030 \\
        \ticker{LSE.L} & 0.19 \pm 0.67 & 30 \pm 450 \\
        \ticker{NOK1V.HE} & -0.15 \pm 1.76 & 20 \pm 330 \\
        \ticker{SAN.MC} & -0.15 \pm 0.73 & 50 \pm 490 \\
        \ticker{VOD.L} & 0.29 \pm 0.50 & 20 \pm 310 \\
        \bottomrule\bottomrule
    \end{tabular}
\end{table}


==> src/tables/consolidated_sarsa.tex <==
\begin{table}[!ht]
    \centering
    \caption{Mean and standard deviation on normalised daily PnL (given in
    units of $10^4$) and mean absolute positions (MAP), with an uncertainty
    given by the max absolute deviation, for a SARSA-based agent using an
    asymmetrically dampened reward function and a linear combination of tile codings
    as the value function approximator.}\label{tab:consolidated:sarsa}

    \begin{tabular}{
        l
        S[table-format=-1.2, table-figures-uncertainty=1,
        separate-uncertainty=true,table-align-uncertainty=true]
        S[table-format=3, table-figures-uncertainty=1,
        separate-uncertainty=true,table-align-uncertainty=true]
    }
        \toprule\toprule
        & {Normalised Daily PnL [$10^{4}$]} & {MAP [units]} \\
        \midrule
        \ticker{CRDI.MI} & 0.03 \pm 0.10 & 1 \pm 2 \\
        \ticker{GASI.MI} & 0.00 \pm 0.22 & 33 \pm 65 \\
        \ticker{GSK.L} & 1.36 \pm 1.33 & 57 \pm 105 \\
        \ticker{HSBA.L} & 3.22 \pm 2.71 & 104 \pm 179 \\
        \ticker{ING.AS} & -1.09 \pm 9.85 & 10 \pm 20 \\
        \ticker{LGEN.L} & 0.93 \pm 1.91 & 229 \pm 361 \\
        \ticker{LSE.L} & 0.34 \pm 0.63 & 72 \pm 139 \\
        \ticker{NOK1V.HE} & -0.95 \pm 6.02 & 31 \pm 62 \\
        \ticker{SAN.MC} & 1.26 \pm 3.08 & 4 \pm 9 \\
        \ticker{VOD.L} & 1.19 \pm 1.51 & 46 \pm 87 \\
        \bottomrule\bottomrule
    \end{tabular}%
\end{table}

